NetFC: enabling accurate floating-point arithmetic on programmable switches

In-network computation has been widely used to accelerate data-intensive distributed applications. Some computational tasks, traditional performed on servers, are offloaded to the network (i.e. programmable switches). However, the computational capacity of programmable switches is limited to simple integer arithmetic operations while many of applications require on-the-fly floating-point operations. To address this issue, prior approaches either adopt a float-to-integer method or directly offload computational tasks to the local CPUs of switches, incurring accuracy loss and delayed processing. To this end, we propose NetFC, a table-lookup method to achieve on-the-fly in-network floating-point arithmetic operations nearly without accuracy loss. NetFC adopts a divide-and-conquer mechanism that converts the original huge table into several much small tables together with some integer operations. NetFC adopts a scaling-factor mechanism for computational accuracy improvement, and a prefix-based lossless table compression method to reduce the memory overhead. We use different types of datasets to evaluate NetFC. The experimental results show that the average accuracy of NetFC can be as high as up to 99.94% at worst with only 448KB memory consumption. Furthermore, we integrate NetFC into Sonata for detecting Slowloris attack, yielding significant decrease of detection delay.

==> introduction/introduction.tex <==
\section{Introduction}
Modern data center operators have to face a challenging task. On the one hand, more and more Internet-scale applications, such as search~\cite{yuan2019distributed}, social networking~\cite{nakajima2020estimating} and e-commerce~\cite{guo2020debiasing}, critically depend on large volumes of data and complicated analysis. On the other hand, they also must satisfy the ever-increasing demand for better response performance. Consequently, large computing and storage resources are consumed to meet the requirement of them.

To fix it, the current contemporary techniques can be classified into two categories: \emph{scale-up} and \emph{scale-out}. The scale-up techniques focus on how to improve the performance of a single device. For example, some devices are often equipped with some special purpose processors to accelerate host-side services~\cite{chen2014diannao,wang2016dlau}. Nonetheless, as the end of Dennard's scaling and Moore's Law are running out of stream, the performance evolution of a single device slows down and is far away from meeting the demands~\cite{2020EFLOPS}. Therefore, the scale-out techniques, such as distributed systems with data parallelism or task parallelism, have widely been proposed~\cite{wen2017terngrad,desai2018compositional}, which utilize a cluster of devices to accelerate the performance of the systems collaboratively. 

% Bottlenecks: network
However, in distributed systems, many applications are data-intensive, which always need frequent communication between each device for exchanging essential data. Unfortunately, this leads to serious communication overhead and their performance is away far from linear speed-up. For example, in some of the FaceBook MapReduce jobs, network communication can occupy up to 70\% of the execution time~\cite{chowdhury2011managing}; or in distributed reinforcement learning, network overhead can be over 80\% of the total cost in each iteration~\cite{li2019accelerating}. In other words, communication often consumes a significant portion of total cost and becomes the performance bottleneck of the systems. This is also echoed by recent literature~\cite{zhang2017poseidon,luo2018parameter}.

% Host-side acceleration
Consequently, many different approaches have been proposed to accelerate network communication for distributed systems. For example, one can design various data compression mechanisms~\cite{alistarh2017qsgd,aji2017sparse} to reduce transmission data volume, but it often incurs additional computation overhead or data loss. Or, one can use RDMA~\cite{guo2016rdma} to replace TCP for speeding up each individual message while RDMA also requires special network supports. Other solutions aiming at mitigating communication burstiness and decreasing the computation waiting time, on the other hand, decouple the dependency between computation and communication via scheduling~\cite{hashemi2018tictac,2019Priority,peng2019generic}. Overall, the above approaches share the same goal - improving the performance from the host side. 

%In-network computation and use case
Recently, a new direction to accelerate distributed systems, \emph{i.e.} in-network computation, has been explored, which considers the network side. Thanks to the development of the network technologies, the network has been equipped with many new devices (e.g. programmable switches~\cite{tofino} and smart network interface~\cite{le2017uno}) so that the network has become capable of providing computational capacity. Consequently, some computational tasks, traditionally performed in the host side, can be offloaded to the network devices. And network traffic can be intercepted and processed by the network devices on the fly based on the pre-offloaded computational logics  before it reaches the hosts. Indeed, researchers in the community has already utilized in-network computation to accelerate different distributed applications and achieve eye-popping performance results. For example, NetCache~\cite{jin2017netcache} is co-designed with programmable switches to achieve more than 2B queries per second, and ATP~\cite{lao2021atp} performs in-network gradient aggregation to improve the training throughput of existing distributed deep learning systems up to 66\%. And Linear-Road~\cite{jepsen2018life}, a steam processing benchmark, shows the capability that achieves 4B events per second.


% Weakness
Unfortunately, the computational capacity of the network is actually very poor. Even the state-of-the-art programmable switches (e.g. Barefoot Tofino~\cite{tofino}) only support simple integer arithmetic operations (e.g. addition and subtraction). This leads to the problem that somewhat complicated tasks either cannot be offloaded to the network for acceleration or seriously decrease other indicator parameters (e.g. accuracy rate). For example, as mentioned before, ATP~\cite{lao2021atp} accelerates distributed deep learning via in-network gradient aggregation, which needs to perform floating-point calculation on programmable switches. To this end, it has to convert floating-point gradients into integer gradients on the host side in advance, but it would lead to serious computation error (see Section~\ref{sec:evaluation}). Let's consider another example. Sonata~\cite{gupta2018sonata} has been designed to achieve network telemetry via programmable switches. Unfortunately, it cannot perform all types of measurement tasks in the data plane, as some of them involve floating-point calculation or division operations. And these operations are not supported by current programmable switches. Instead, it has to mirror the corresponding network traffic to the steam processor for further processing, which inevitably introduces additional latency. Overall, the poor computational capacity of the network barriers the in-network acceleration.

% Our work
To address this challenge, we design a novel approach --- NetFC in this paper to enhance the computational capacity of programmable switches. Equipped with our NetFC, we can perform not only floating-point calculations but also complex multiply-divide operations in programmable switches. Specifically, NetFC maps floating-point numbers into logarithm number system to simplify the representation of data, and then further converts floating-point calculation into multiple table-lookup operations. To reduce the overhead of NetFC, we also further propose a mask-based approach to reduce the memory usage by NetFC. With the experiments under three different types of datasets, we show that the middle value of the computational accuracy of NetFC can be achieved up to 100\%, which is much better than the baseline, the floating-to-integer solution (36.79\% computational accuracy at worst). In addition, we further implement an use cases to demonstrate the efficiency of our NetFC.

To sum up, the contributions of this paper are three-fold:
\begin{itemize}
  \item To enhance the computational capacity, we propose a table-up approach, NetFC, to achieve floating-point calculation in programmable switches. 

  \item To mitigate the overhead introduced by our NetFC, we propose a mask-based approach to reduce the size of floating-point calculation tables. Furthermore, we design a scaling factor algorithm to improve the computational accuracy. 
  
  \item We implement NetFC based on Barefoot Tofino switches. With three different types of datasets, we show that our NetFC can achieve high computational accuracy and low on-chip memory usage. In addition, we further implement an use cases to demonstrate its efficiency.
\end{itemize} 

The remainder of this paper is organized as follows. Section~\ref{sec:background} describes the background and the motivation. We present the design of our NetFC and its fundamental theory in Section~\ref{sec:design}. Section~\ref{sec:imple} shows the implementation details and our optimization mechanism. We evaluate our NetFC in Section~\ref{sec:evaluation} and present an use cases that are equipped with our NetFC in Section~\ref{sec:usecase}. We finally discuss the related work in Section~\ref{sec:related} and concludes our work in Section~\ref{sec:conclusion}.




